Homogenisation for the monodomain model in the presence of microscopic fibrotic structures

Computational models in cardiac electrophysiology are notorious for long runtimes, restricting the numbers of nodes and mesh elements in the numerical discretisations used for their solution. This makes it particularly challenging to incorporate structural heterogeneities on small spatial scales, preventing a full understanding of the critical arrhythmogenic effects of conditions such as cardiac fibrosis. In this work, we explore the technique of homogenisation by volume averaging for the inclusion of non-conductive micro-structures into larger-scale cardiac meshes with minor computational overhead. Importantly, our approach is not restricted to periodic patterns, enabling homogenised models to represent, for example, the intricate patterns of collagen deposition present in different types of fibrosis. We first highlight the importance of appropriate boundary condition choice for the closure problems that define the parameters of homogenised models. Then, we demonstrate the technique's ability to correctly upscale the effects of fibrotic patterns with a spatial resolution of 10 $\mu$m into much larger numerical mesh sizes of 100-250 $\mu$m. The homogenised models using these coarser meshes correctly predict critical pro-arrhythmic effects of fibrosis, including slowed conduction, source/sink mismatch, and stabilisation of re-entrant activation patterns. As such, this approach to homogenisation represents a significant step towards whole organ simulations that unravel the effects of microscopic cardiac tissue heterogeneities.

==> commands.tex <==
\newcommand{\pde}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdeb}[1]{\frac{\partial}{\partial #1}}
\newcommand{\pden}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}
\newcommand{\pdebn}[2]{\frac{\partial^{#2}}{\partial #1^{#2}}}
\newcommand{\de}[2]{\frac{d #1}{d #2}}
\newcommand{\deb}[1]{\frac{d}{d #1}}
\newcommand{\den}[3]{\frac{d^{#3} #1}{d #2^{#3}}}
\newcommand{\debn}[2]{\frac{d^{#2}}{d #1^{#2}}}
\newcommand{\refer}[1]{[\ref{#1}]}
\newcommand{\figref}[1] {Figure \ref{#1}}
\newcommand{\tabref}[1] {Table \ref{#1}}
\newcommand{\erfc}[1]{\mathrm{erfc}\left(#1\right)}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
